CloudHealth: A Model-Driven Approach to Watch the Health of Cloud Services

Cloud systems are complex and large systems where services provided by different operators must coexist and eventually cooperate. In such a complex environment, controlling the health of both the whole environment and the individual services is extremely important to timely and effectively react to misbehaviours, unexpected events, and failures. Although there are solutions to monitor cloud systems at different granularity levels, how to relate the many KPIs that can be collected about the health of the system and how health information can be properly reported to operators are open questions. This paper reports the early results we achieved in the challenge of monitoring the health of cloud systems. In particular we present CloudHealth, a model-based health monitoring approach that can be used by operators to watch specific quality attributes. The CloudHealth Monitoring Model describes how to operationalize high level monitoring goals by dividing them into subgoals, deriving metrics for the subgoals, and using probes to collect the metrics. We use the CloudHealth Monitoring Model to control the probes that must be deployed on the target system, the KPIs that are dynamically collected, and the visualization of the data in dashboards.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> discussion.tex <==
\section{discussion}
\label{sec:discussion}

%\leonardo{The content of this section makes a lot of sense, but most of the paragraphs can be moved elsewhere or merged with other paragraphs.}
The first step consists of identifying the monitoring goals. 
We started from a sound definition of quality demands that is reported in the ISO/IEC TS 25011:2017 standard. 
The standard reports a number of meaningful quality features that are relevent when it comes to guarantee a given 
quality standard both for products and services.  
As can be seen by comparing the original standard to reported in Table \ref{table:monitoring-goals-definitions} we isolated a subset of quality properties of a cloud systems, based on our experience on cloud systems.

The selection process become even more critical because usually there are manyfold interests that take place in a complex management scenario such as that of a large cloud infrastructure. When it comes to find a trade off between different stakeholders, namely all the various subjects involved in the cloud infrastructure management who might have different perspective, approaches, and interests in the way the health of the system is achieved.
	%
	%Put in other words, the various stakeholders, namely the different subjects involved in infrastructure management have different perspective, approaches, and interests. 
	This might be potentially reflected in the different monitoring strategies proposed, thus a trade-off has to be reached to 	resolve the mismatch between conflicting proposals. \leonardo{We have to be careful when we mention this argument about multiple interests. We do not do anything to solve conflicts.}
%For many reasons it is need to find a trade off between the different solutions. 

We consider that cloud management might benefit by the adoption of CloudHealth in several respect. 
	\begin{itemize}
		\item By providing a common language (and a global picture), CloudHealth is likely to enahnce the communication between the stakeholder, mitigating the risk of misunderstanding.
		\item CloudHealth structure the monitoring goals in a hierarchical structure, where we can distinguish elements at different levels of abstraction (i.e., main-goals, sub-goals, etc.). Different stakeholder might locate themselves better suited to "speak the language" appropriate to a given layer. The presented "taxonomy" spans from a more abstract to the a more implementative one.
	\end{itemize}
	
To a certain extent CloudHealth might look like a Performance Monitoring System (PMS), which are traditionally aimed
	at keeping track of the process performance and quality in business process \cite{(Evans:2004)}
	One of the most difficult aspect in desining such a kind of model is to find an appropriate appropriate set of
	indicators to proper represent the system under monitoring \cite{Franceschini:2006b}.


==> todo-section.tex <==
\section*{TODO}
\label{sec:todo}

This Section is for internal use only and it is going to die before the submission. 
It collects comments and TODOs from
the authors.

\textbf{MAT}

\begin{itemize}
	\item separate paragraph in different files (using input command) to enhance the mantainability and reduce the occurrence of conflicts.
	\item I'm not sure if I understand what can be a running example at this stage. The computation of the throughput, maybe?
	\item About the name, what do you think of MEALS: Monitoring hEAlth in cLoud Systems? We can also say Quality Meal \dots
	\item I think there are at least few missing points at this stage.
	\begin{enumerate}
	\item Let's say I'm a manager or other IT guy (a decision maker) who wants to define some goals in terms of system health. In which way this can be done? From an operative perspective I assume there would be a dashboard. However:\\
	\begin{enumerate}
		
	\item How can this be performed? For example, I have accuracy: how I can decide that my system needs more accuracy? What accuracy means for me/in a specific case.
	
	\item In our framework, are we providing a way to associate goals to other KPI? Or it is stuck to the ISO standard?
	\end{enumerate}

	\item I think we need to provide a definition/distinction about these goals. I think that is intuitive what business goals might be (i.e. More customers, more sells, etc.). At the same time,  it is less clear what healing goals are and how to relate them to the business goals (if this is the case).
	
	\item For any step of the process we should provide some hints on how can be implemented, whether it is ad hoc (using general language or DSLs?) or by leveraging existing solutions. Also it can be useful to provide some info about the formalism (is the tree represented as a XML configuration file, etc.)
	Can we consider Ansible a good candidate to take care of part of this process? Just to get real with our arguments.
	
	
	\item We should converge on what is the basic definition of our proposal: tool, model, framework (more things together)? 
	
	\item Elaphant in the room. What if someone else proposed (or even implemented) already something similar?
	
\end{enumerate}
\end{itemize}

\textbf{LEO}
\begin{itemize}
	\item In the introduction I would also mention the complexity of handling probes (deploy and undeploy them from a running system) as part of the motivation
	\item I propose to give a name to our framework and use it as title for section 2.
	
	\item Handling probes is not a tool aspect only, but requires a proper solution to map metrics to both the corresponding probes and entities to be monitored. So I would include a subsection to discuss this.
	\item If Discussion is gonna be discussion of use cases, which to me is a good idea, I would change the name of the section into Use Cases.
	\item If possible, I would use a running example to present the approach.
\end{itemize}

